Conjugate heat transfer in turbulent pipe flow with azimuthally non-uniform heating

Turbulent conjugate heat transfer (CHT) in pipes with azimuthally non-uniform heating is studied theoretically and numerically with a focus on low-$\mathrm{Pr}$ fluids. While the influence of the solid properties is well documented for uniform heat flux, their effect under azimuthally non-uniform heating has not been explored systematically. We address this gap by combining spectral analysis of the problem -- which reduces arbitrary boundary conditions to a discrete set of azimuthal wavenumbers -- with well-resolved numerical simulations of thermally and hydraulically fully developed turbulent pipe flow at $\mathrm{Re}_\tau \approx 180$ for $\mathrm{Pr} = \{0.025, 0.71\}$, representative of liquid metals and air. Two principal results emerge: (i) the global Nusselt number is independent of the azimuthal heat-flux distribution and exhibits only a minor dependence on the solid properties, resolving an open question for low-Prandtl-number fluids; (ii) CHT nevertheless strongly affects the azimuthally resolved mean temperature at low $\mathrm{Pr}$, where azimuthal conduction in the solid homogenises the interface heat flux, and governs the level of temperature fluctuations through the effusivity ratio (thermal activity ratio) $K$. Finally, an analysis of the turbulent Prandtl number $\mathrm{Pr}_{t}$ shows a strong anisotropy, particularly near the wall, and a dependence on the azimuthal wavenumber.

==> figures/pipe/sketch.tex <==
\pgfdeclarelayer{background}
\pgfdeclarelayer{foreground}
\pgfsetlayers{background,main,foreground}

\newcommand{\drawbasepipetwo}[1]{
	\fill[#1] (90:0.5)  ++ (2, 0)  arc  (90:-90:4mm and 5mm) -- ++ (2, 0) arc  (-90:90:4mm and 5mm);
	
	\fill[white] (90:0.5)  arc  (90:-90:4mm and 5mm) -- ++ (2, 0) arc  (-90:90:4mm and 5mm);
	
	\draw[black!20,] (4, 0) ++ (90:4mm and 5mm) arc  (90:270:4mm and 5mm);
	
	\draw[black!20,] (90:0.5) ++ (2, 0) arc  (90:270:4mm and 5mm);
	
	\begin{pgfonlayer}{foreground}
		\draw[](0, 0) ellipse(4mm and 5mm);
		\draw (90:0.5)  ++ (2, 0)  arc  (90:-90:4mm and 5mm);
		\draw[->] (2, 0) -- node[above left=-0.1cm] {$z$} ++ (0.3, 0) ;
		
	\end{pgfonlayer}
	\draw (90:0.5) -- ++ (4, 0)  arc  (90:-90:4mm and 5mm) -- ++ (-4, 0);
	
	
	\draw[](2, 0) ellipse(0.4mm and 0.5mm);
	
	\draw (0, -0.25) to[out=-180, in=45] ++ (200:0.5) node[below] {$T_0$};
	
	\draw[->]  (-0.5, 0) node[below left=-0.1cm] {$u_z(r)$} --  (0, 0) ;
}




\newcommand{\drawenvelope}[4]{
	
	\edef\onEllipse{\noexpand\pgfpointpolar{\phi}{4mm and 5mm}}
	\edef\outerEllipse{\noexpand\pgfpointpolar{\phi}{1mm and 1.2mm}}
	\foreach \phi in {#1} {
		\pgfmathparse{#4(#1)}  
		\let\y\pgfmathresult 
		\pgfpathmoveto{\onEllipse}
	}
	
	\foreach \phi in {#1, #2, ..., #3} {
		\pgfmathparse{#4(\phi)}  
		\let\y\pgfmathresult 
		
		
		\ifdim \y pt = 0 pt
		\pgfpathmoveto{\onEllipse}
		\else
		\pgfpathlineto{\pgfpointadd{\onEllipse}{\pgfpointscale{\y}{\outerEllipse}}}
		\fi
		
	}
	\color{red}
	\pgfusepath{draw}
}
\newcommand{\drawpipeheated}[1]{
	
	\begin{pgfonlayer}{background}
		\draw[overlay, fill=white, decorate, decoration=example, line join=bevel] (0, -0.5) -- ++(-2.01, 0);
		\draw[overlay, fill=white, decorate, decoration=example, line join=bevel] (2.0, 0.5) -- (4.02, 0.5);
	\end{pgfonlayer}
	\draw (1, -0.5) to[out=-45, in=135] ++(0, -0.4) node[right] {adiabatic};
	
	%
	\foreach \z in {2, 2.4, ..., 4}{
		
		
		\begin{scope}[xshift=\z cm]
			\drawenvelope{-90}{-89}{90}{#1}
			\begin{pgfonlayer}{background}
				\drawenvelope{90}{91}{270}{#1}
			\end{pgfonlayer}
		\end{scope}
		
		\foreach \phi in {-90, -75, ..., 90}{
			\pgfmathparse{#1(\phi)}
			\let\y\pgfmathresult
			
			\ifdim \y pt = 0 pt
			\else
			\draw[{Stealth[scale={\y}, length=0.5mm,width=0.5mm]}-] (\z, 0) ++ (\phi:4mm and 5mm) -- ($(\z, 0) +
			(\phi:4mm and 5mm) + #1(\phi)*(\phi:1mm and 1.2mm)$);
			\fi
			
			\pgfmathparse{#1(\phi+180)}
			\let\y\pgfmathresult
			
			\ifdim \y pt = 0 pt
			\else
			\begin{pgfonlayer}{background}
				\draw[{Stealth[scale={\y}, length=0.5mm,width=0.5mm]}-] (\z, 0) ++ (\phi+180:4mm and 5mm) -- ($(\z, 0) + #1(\phi+180)*(\phi+180:5mm and 6.2mm)$);
			\end{pgfonlayer}
			\fi
			
			
		}
}}

\pgfmathdeclarefunction{const}{1}{%
	\pgfmathparse{1}
}
\pgfmathdeclarefunction{halfsin}{1}{%
	\pgfmathparse{max(sin(#1+50), 0)*1}%
}
\pgfdeclarehorizontalshading{grad3}{3cm}{
	color(0cm)=(black);
	color(0.3cm)=(black!40);color(0.8cm)=(white);
	color(1cm)=(white)
}


\begin{figure}
	\centering
	\begin{subfigure}[b]{0.48\textwidth}
		\centering
		\tikzsetnextfilename{pipe-sketch-graetz-dirichlet}
		\begin{tikzpicture}
			\begin{scope}[rotate=50]
				\drawbasepipetwo{black!10}
				\draw (3, -0.5) to[out=-45, in=135] ++(0, -0.4) node[right] {$T_1$};
				\draw (1, -0.5) to[out=-45, in=135] ++(0, -0.4) node[right] {$T_0$};
			\end{scope}
		\end{tikzpicture}
		\caption{Graetz problem with Dirichlet boundary conditions}
		\label{fig:pipe_isothermal}
	\end{subfigure}
	\hfill
	\begin{subfigure}[b]{0.48\textwidth}
		\centering
		\tikzsetnextfilename{pipe-sketch-graetz-neumann}
		\begin{tikzpicture}
			\begin{scope}[rotate=50]
				
				\drawbasepipetwo{black!30}
				\drawpipeheated{const}
				\draw (3, -0.5) to[out=-45, in=135] ++(0, -0.4) node[right, align=left] {uniform \\ heating};
				\draw (3, 0.8) node[red] {$q$};
			\end{scope}
		\end{tikzpicture}
		\caption{Graetz problem with homogeneous Neumann boundary conditions}
		\label{fig:pipe_homogeneous}
	\end{subfigure}
	\\
	
	\begin{subfigure}[b]{0.48\textwidth}
		\centering
		\tikzsetnextfilename{pipe-sketch-graetz-neumann-inhom}
		\begin{tikzpicture}
			\begin{scope}[rotate=50]
				
				\drawbasepipetwo{shading=grad3, shading angle=-50}
				\drawpipeheated{halfsin}
				\draw (3, -0.5) to[out=-45, in=135] ++(0, -0.4) node[right, align=left] {non-uniform \\ heating};
				\draw[red] (2, 0) ++ (-50:4mm and 5mm) -- ++ (2, 0);
				\draw (3, 0.9) node[red] {$q(\phi)$};
				
				\draw[->] (-90:2mm and 2.5mm) ++ (2, 0) arc  (-90:-220:2mm and 2.5mm) node[pos=0.5, below left=-0.1cm] {$\phi$};
			\end{scope}
			\begin{scope}[xshift=2cm, yshift=9cm]
				\draw[fill=yellow] (250:4) arc (250:290:4); 
				\foreach \phi in {255, 265, ..., 285}{
					\draw[yellow, line width=0.05cm] (\phi:4.2) -- ++(0, -1);
				}
			\end{scope}
		\end{tikzpicture}
		\caption{Graetz problem with inhomogeneous Neumann boundary conditions}
		\label{fig:pipe_inhomogeneous}
	\end{subfigure}
	\hfill
	\begin{subfigure}[b]{0.48\textwidth}
		\centering
		
		\def\majorinner{3}
		\def\minorinner{2.4}
		\tikzsetnextfilename{pipe-sketch-graetz-neumann-inhom-conj}
		\begin{tikzpicture}
			\def\innerellipse{(\minorinner mm and \majorinner mm)}
			\def\innerellipsea{\minorinner mm and \majorinner mm}
			\begin{scope}[rotate=50]
				\drawbasepipetwo{shading=grad3, shading angle=-50}
				\draw[densely dashed, black!20] (90:\majorinner mm) -- ++ (4, 0)  arc  (90:-90:\innerellipsea) -- ++ (-4, 0);
				\draw[densely dashed, black!20] (4, 0) ++ (90:\innerellipsea) arc  (90:270:\innerellipsea);
				
				\draw[densely dashed, black!20] (90:\majorinner mm)  ++ (2, 0)  arc  (90:-90:\innerellipsea);
				\draw[densely dashed, black!20] (90:\majorinner mm) ++ (2, 0) arc  (90:270:\innerellipsea);
				
				
				\fill[even odd rule, pattern=north east lines] (0,0) ellipse (4mm and 5mm) ellipse \innerellipse ;
				\fill[even odd rule, pattern=north east lines, pattern color=black!10] (2,0) ellipse (4mm and 5mm) ellipse \innerellipse ;
				\fill[even odd rule, pattern=north east lines, pattern color=black!10] (4,0) ellipse (4mm and 5mm) ellipse \innerellipse ;
				\draw[](0, 0) ellipse \innerellipse;
				
				
				
				\drawpipeheated{halfsin}
				\draw (3, -0.5) to[out=-45, in=135] ++(0, -0.4) node[right, align=left] {non-uniform \\ heating};
				\draw[red] (2, 0) ++ (-50:4mm and 5mm) -- ++ (2, 0);
				
				\draw (0, 0.4) to[out=-180, in=-45] ++ (150:0.5) node[left] {solid};
				
				\draw (3.5, 0.9) node[red] {$q(\phi)$};
				
				\draw[->] (-90:2mm and 2.5mm) ++ (2, 0) arc  (-90:-220:2mm and 2.5mm) node[pos=0.5, below left=-0.1cm] {$\phi$};
			\end{scope}
			\begin{scope}[xshift=2cm, yshift=9cm]
				\draw[fill=yellow] (250:4) arc (250:290:4); 
				\foreach \phi in {255, 265, ..., 285}{
					\draw[yellow, line width=0.05cm] (\phi:4.2) -- ++(0, -1);
				}
			\end{scope}
			\begin{scope}[yshift=4cm, xshift=-1cm, scale=1]
				\draw[pattern=north east lines, even odd rule] (0, 0) circle (1) circle (0.6);
				\fill (0, 0) circle (0.05);
				\draw[->] (0, 0) -- node[below right=-0.1cm, pos=0.4] {$R_i$} ++ (45:0.6);
				\draw[->] (0, 0) -- node[below left=-0.15cm, pos=0.2] {$R_o$} ++ (135:1);
				\draw (0, -0.3) to[out=-90, in=90] ++ (0.5, -0.8) node[below, xshift=0.5cm, align=left] {$\rho_f, c_{p, f}, \lambda_f$};
				\draw (-110:0.8) to[out=-90, in=90] (-0.5, -1.6) node[below, xshift=0.5cm, align=left] {$\rho_s, c_{p, s}, \lambda_s$};
			\end{scope}
		\end{tikzpicture}
		\caption{Conjugated Graetz problem with inhomogeneous Neumann boundary conditions}
		\label{fig:pipe_inhomogeneous_cht}
	\end{subfigure}
	
	\caption{Sketch of the typical configurations of the Graetz problem (\cref{fig:pipe_isothermal,fig:pipe_homogeneous}), as well as the non-uniform heating case and conjugated case considered in this chapter. Adapted from \cite{neuhauserSolutionExtendedGraetz2025}.}
	\label{fig:sketch_pipe}
\end{figure}


==> nudecomp-azimuthal.tex <==
%

\textcolor{red}{TODO: Decide whether we want to keep this in. Then we need to add the derivation for this specific case.
}


The local Nusselt number, as defined by \cref{eq:nulocal_def}, can be evaluated for each wavenumber $k$. In the given setting, it can be understood as a measure of how uniform the (modal) temperature profile is within the pipe. It aggregates the effect of all heat transfer mechanisms, i.e.\ radial and azimuthal transport, due to both mean conduction and turbulent diffusion. \Cref{plot:nuvalues} displays $\Nu_l$ for the wavenumbers considered. After a global minimum at $k=1$, $\Nu_l$ increases monotonically in $k$, approximately linear with slope $\dv*{\Nu_l}{k} \approx 2$, equal for all considered cases.\footnote{For reference, $\Nu_l = 2k + 16 / (k+6)$ for $k > 0$, $48/11$ otherwise for laminar flow.}

While $\Nu_l$ aggregates all heat transfer mechanisms, the decomposition derived in \cref{sec:nudecomp} provides insight into the relative importance of the various heat transfer mechanisms. \Cref{plot:nudecomp:pr0.025,plot:nudecomp:pr0.71} display the individual contributions to the decomposition \cref{eq:nudecomp2} for $k=0..10$. The term $\Nu_{lam} / \Nu_{RSS}$ depends only on the turbulent velocity profile (fixed for a given $\Re_\tau$). It is therefore essentially independent of $\Pr$ and $k$ (the $k=0$ term differs because of the mean temperature forcing). For uniform heating ($k=0$), turbulent mixing is stronger for $\Pr=0.71$ than for $\Pr=0.025$. Consequently, $\Nu_{lam} / \Nu_{HF,r}$ is larger, and thus the overall Nusselt number $\Nu_l$ (which coincides with $\Nu$ at $k=0$) increases. 

\input{figures/pipe/nudecomp}

For $\Pr = 0.025$, the contribution associated with azimuthal conduction increases with $k$, while the radial and turbulent heat flux terms remain small. Hence the rise of $\Nu_l$ is primarily driven by molecular conduction in the azimuthal direction. For $\Pr = 0.71$, the azimuthal conduction term also grows with $k$, but is dominated by turbulent azimuthal transport, which appears to saturate at higher $k$. At low $k$, radial turbulent transport contributes significantly, but its relative importance diminishes as $k$ increases. 

In summary, the decomposition of $\Nu_l$ highlights distinct heat transfer mechanisms under non-uniform heating. For the low-$\Pr$ fluid, the main transport mechanism at this $\Re_b$ is azimuthal molecular conduction. For $\Pr=0.71$, the main driver of azimuthal transport is turbulence, while radial (turbulent) transport is only important at low wavenumbers. For both $\Pr$ numbers, the relative importance of azimuthal transport through molecular diffusion increases with $k$ compared to azimuthal transport through turbulent heat flux.

